Multi-Task Learning for Visual Scene Understanding

Despite the recent progress in deep learning, most approaches still go for a silo-like solution, focusing on learning each task in isolation: training a separate neural network for each individual task. Many real-world problems, however, call for a multi-modal approach and, therefore, for multi-tasking models. Multi-task learning (MTL) aims to leverage useful information across tasks to improve the generalization capability of a model. This thesis is concerned with multi-task learning in the context of computer vision. First, we review existing approaches for MTL. Next, we propose several methods that tackle important aspects of multi-task learning. The proposed methods are evaluated on various benchmarks. The results show several advances in the state-of-the-art of multi-task learning. Finally, we discuss several possibilities for future work.

==> chapters/abstract/abstract.tex <==
% !TeX root = ../../thesis.tex
\chapter{Abstract}
\label{ch:abstract}
Despite the recent progress in deep learning, most approaches still go for a silo-like solution, training a separate neural network for each individual task. Yet, many real-world problems require to solve a multitude of tasks concurrently. For example, an autonomous vehicle should be able to detect all objects in the scene, localize them, estimate their distance and trajectory, etc., in order to safely navigate itself in its surroundings. Similarly, an image recognition system for commerce applications should be able to tag products, retrieve similar items, come up with personalized recommendations, etc., to provide customers with the best possible service. These types of problems have motivated researchers to build multi-task learning models.

The key idea of multi-task learning is to learn multiple tasks in parallel while sharing the learned representations. Multi-task networks bring several practical advantages compared to the single-tasking case, where each individual task is solved separately by its own network.  First, due to the sharing of layers, the resulting memory footprint is substantially reduced. Second, as they avoid to repeatedly calculate features in the shared layers, once for every task, they show increased inference speeds. Third, they have the potential to improve the performance if the associated tasks share complementary information, or act as a regularizer for one another. 

We are faced with two important challenges when building multi-task learning models. First, we need to come up with neural network architectures that can handle multiple tasks. Second, we need to develop novel training recipes for jointly learning the tasks. In particular, since we are optimizing for multiple objectives in parallel, one or more tasks could start to dominate the weight update process, hindering the model from learning the other tasks. In this manuscript, we delve into both problems within the context of visual scene understanding. 

We propose two new types of models to address the architectural problem. First, we explore branched multi-task networks, where the deeper layers of the neural network gradually grow more task-specific. We introduce a principled method to automate the construction of such branched multi-task networks. The construction process groups together the tasks that can be solved with a similar set of features, while making a trade-off between task similarity and network complexity. In this way, our method produces models that yield a better trade-off between the performance and the amount of computational resources. 

Second, we propose a novel neural network architecture for jointly tackling multiple dense prediction tasks. The key idea is to improve the predictions for each task by distilling useful information from the predictions of other tasks at \emph{multiple scales}. The motivation for including multiple scales is based upon the observation that tasks with high affinity at a certain scale are not guaranteed to retain this behavior at other scales, and vice versa. Extensive experiments across two popular benchmarks for dense labeling show that, unlike prior work, our model delivers on the full potential of multi-task learning, that is, smaller memory footprint, reduced number of calculations, and better performance w.r.t. single-task learning. 

Further, we also consider the multi-task learning optimization problem. We first analyze several existing techniques for balancing the learning of tasks. Surprisingly, we uncover several discrepancies between works. We hypothesize that this can be attributed to the lack of standardized benchmarks for multi-task learning, and different benchmarks benefit from a specific strategy. Based upon this result, we then isolate the elements that are most promising and propose a set of heuristics to balance the tasks. The heuristics are of practical nature, and result in more robust performance across different benchmarks.

In the final chapter, we consider the problem of scene understanding from an alternative point-of-view. Many of the models described in the literature benefit from supervised pretraining. In this case, the model is first pretrained on a larger annotated dataset like ImageNet, before being transferred to the tasks of interest. This allows the model to perform well, even on datasets with only a modest amount of labeled examples. Unfortunately, supervised pretraining relies on an annotated dataset itself, which limits it's applicability. To address this problem, researchers started to explore self-supervised learning methods. We revisit recent popular works based upon contrastive learning. First, we show that an existing method like MoCo obtains robust results across different datasets, including scene-centric, long-tailed and domain-specific data. Second, we improve the learned representations by imposing additional invariances. This result directly benefits many downstream tasks like semantic segmentation, detection, etc. Finally, we show that the improvements obtained via self-supervised learning translate to multi-task learning networks too. 

In summary, this manuscript presents several important contributions that improve multi-task learning models for visual scene understanding. The innovations focus on improving the neural network architecture, the optimization process and the pretraining aspect. All methods are thoroughly tested across a variety of benchmarks. The code is made publicly available: \url{https://github.com/SimonVandenhende}.

==> chapters/abstractnl/abstractnl.tex <==
% !TeX root = ../../thesis.tex
\chapter{Beknopte samenvatting}
\label{ch:abstractnl}
Ondanks de recente vooruitgang in \emph{machine learning}, gesterkt door het gebruik van diepe neurale netwerken, worden modellen nog steeds gebouwd voor individuele taken. Hierbij wordt een apart neuraal netwerk getraind voor elke taak. Vele praktische problemen vereisen echter dat we verschillende taken synchroon uitvoeren. Om bijvoorbeeld veilig te kunnen navigeren moet een autonoom voertuig gelijktijdig alle objecten in de sc\`ene detecteren, hun locatie bepalen, de afstand schatten, etc. Op gelijkaardige wijze moet een intelligent systeem voor commerci\"ele applicaties producten herkennen, gelijkaardige items ophalen, persoonlijke aanbiedingen voorstellen, etc. Dit om klanten de beste mogelijke ervaring te bieden. Om dergelijke problemen op te lossen begonnen onderzoekers  aan de de bouw van \emph{multi-task learning} modellen die meerdere taken gelijktijdig kunnen uitvoeren.

Het idee achter \emph{multi-task learning} is om meerdere taken in parallel te leren, terwijl de geleerde representaties gedeeld worden tussen taken. In vergelijking met het afzonderlijk afhandelen van elke taak bieden \emph{multi-task learning networks} verschillende praktische voordelen. Ten eerste laat het delen van de representaties toe om minder computergeheugen te gebruiken. Verder kan een deel van de berekeningen afgeschreven worden over meerdere taken, wat de totale hoeveelheid rekenwerk vermindert. Tenslotte verbetert ook de performantie wanneer taken informatie kunnen uitwisselen.

Er zijn een aantal uitdagingen voor het bouwen van \emph{multi-task learning} modellen. Allereerst moeten we nieuwe neurale netwerkarchitecturen bedenken die geschikt zijn voor het behandelen van meerdere taken. Ten tweede moeten we optimalisatietechnieken ontwikkelen die toelaten om het model meerdere taken in parallel aan te leren. Een uitdaging hierbij is dat een enkele of meerdere taken het leerproces kunnen domineren en het model bijgevolg niet in staat is om de resterende taken te leren. In deze thesis behandelen we beide uitdagingen binnen de context van \emph{visual scene understanding.}

We stellen twee nieuwe neurale netwerk architecturen voor. Ten eerste bestuderen we \emph{branched multi-task networks}, waar de diepere lagen van het neurale netwerk gradueel meer taakspecifiek worden. We introduceren een nieuw algoritme voor de automatische constructie van dergelijke netwerken. Het algoritme groepeert taken die opgelost kunnen worden aan de hand van een gelijkaardige verzameling visuele kenmerken. Tegelijkertijd brengen we ook de complexiteit van het neurale netwerk in rekening. De modellen gegenereerd met onze methode realiseren een betere trade-off tussen de performantie en de benodigde rekenkracht. Dit wordt duidelijk aangetoond in onze experimentele resultaten. 

Het tweede model dat we voorstellen focust expliciet op meerdere per-pixel-taken. Het idee is om de predicties voor elke taak te verbeteren door informatie te halen uit de predicties van andere taken. We passen dit principe toe op meerdere schalen nadat we via observatie hebben geconstateerd dat de geometrische relaties tussen taken wijzigen afhankelijk van de gebruikte schaal. Op deze wijze halen we de maximale hoeveelheid informatie uit andere taken voor het verbeteren van de predicties. De experimentele resultaten tonen aan dat ons model beter presteert met betrekking tot de hoeveelheid computergeheugen, het aantal bewerkingen en de performantie. 

We  onderzoeken ook het \emph{multi-task-learning-optimalisatieprobleem}. Eerst voeren we een vergelijkende studie uit van bestaande werken. Tot onze verbazing  ontdekken we verschillende discrepanties tussen bestaande werken. De verklaring hiervoor is dat  de methodes ontwikkeld werden voor een specifieke dataset of toepassing. Gebaseerd op dit resultaat proberen we de meest veelbelovende elementen te isoleren en stellen we een aantal heuristieken voor. De heuristieken zijn praktisch geori\"enteerd. Verder tonen we aan dat het gebruik van heuristieken zich vertaalt in meer robuuste resultaten.

In het laatste hoofdstuk  onderzoeken we het probleem van \emph{visual scene understanding} vanuit een alternatief oogpunt. Veel modellen maken gebruik van gesuperviseerd pretrainen. Hierbij wordt het model eerst  getraind op een andere, grotere dataset, waarna de gewichten overgedragen worden naar de taak waarin we ge\"interesseerd zijn. Dit laat toe om een hoge performantie te behalen, zelfs op datasets met slechts een beperkte hoeveelheid  gelabelde voorbeelden. Gesuperviseerd pretrainen maakt echter zelf gebruik van een gelabelde dataset en dit beperkt het gebruik. Onderzoekers werken daarom op zelf-gesuperviseerde methodes, waarbij het leersignaal vanuit de data zelf komt. We bestuderen recente methodes gebaseerd op \emph{contrastive learning}. Eerst tonen we aan dat een bestaande methode zoals \emph{MoCo} robuuste resultaten kan behalen voor verscheidene datasets - waaronder \emph{scene-centric}, ongebalanceerde en domeinspecifieke datasets. Verder verbeteren we de representaties door extra invarianties op te leggen. Dit resultaat laat toe bestaande modellen voor segmentatie, objectdetectie, etc. te verbeteren. Tenslotte tonen we aan dat we op een gelijkaardige manier ook de performantie van \emph{multi-task learning} modellen kunnen verbeteren.

Deze thesis beschrijft verschillende methodes voor het verbeteren van \emph{multi-task learning} modellen voor \emph{visual scene understanding}. De contributies focussen op het verbeteren van de netwerkarchitectuur, het optimalisatieproces en het pre-trainingsaspect. Alle innovaties werden getest op verschillende datasets. De bijhorende code is publiek beschikbaar: \url{https://github.com/SimonVandenhende}.

\cleardoublepage




==> chapters/curriculum/curriculum.tex <==
% !TeX root = ../../thesis.tex
\chapter{Curriculum}
\label{ch: curriculum}
Simon Vandenhende was born in Roeselare, Belgium in 1995. He received his bachelor's and master's degree in Electrical Engineering from KU Leuven. During his master's, he worked as an intern at the SI2 lab, NCTU, Taiwan. Later on, Simon developed a strong interest in machine learning and computer vision. This led him to join the VISICS computer vision lab at KU Leuven in 2017 to pursue a PhD under the supervision of Prof. Luc van Gool. His research focuses on multi-task learning and self-supervised representation learning. In 2019, Simon won a best paper award at the International Conference on Machine Vision Applications. He also co-organized workshops on multi-modal learning and multi-task learning at ECCV'20 and ICCV'21 respectively. In Fall 2021, he participated in a research internship at Facebook AI Research (FAIR). 

\cleardoublepage

==> chapters/preface/preface.tex <==
% !TeX root = ../../thesis.tex
\chapter*{Preface}
\label{ch:preface}
A PhD is more than just another university degree. A PhD is about the pursuit of knowledge, the aspiration to figure things out and the love to explore new ideas. It is a personal journey filled with challenges, discoveries and encounters with extraordinary people. As I reflect on this incredible adventure, a feeling of great contentment prevails. Now all that rests is to thank my collaborators, colleagues, friends and family members for helping me to achieve my goals.

I wish to start by thanking my advisor Luc Van Gool for taking me on board as one of his PhD students. Luc, thank you for our discussions, for putting your trust in me even when things did not go according to plan and for all the freedom in research you provided. You created a unique place where I could freely pursue my research interests without distractions. The environment you provided allowed me to turn my ideas into reality and push my research further than what I hoped for. Despite all your accomplishments in research, you were always down-to-earth and ready to hear out my opinion. I am most honored that you chose to advise me. 

I am thankful for the members of my supervisory committee Prof. Tinne Tuytelaars, Prof. Marie-Francine Moens and Prof. Matthew Blaschko for providing me with feedback and support throughout the years. Further, I would like to thank Prof. Hakan Bilen and Prof. Gemma Roig for promptly agreeing to serve on my examination committee. Also, I thank Prof. Paul Sas for serving as a chair. 

This manuscript would have never been in its current state without the guidance of Dr. Stamatios Georgoulis, who took me under his wings when I started my PhD. Stam, thank you for acting as a mentor, for believing in me, for having countless meetings with me, for sharing your knowledge with me, and for teaching me how to write papers. It is hard to put into words the gratitude that I feel for the endless support you gave me. I hope we can meet again soon!

Another remarkable colleague was Wouter Van Gansbeke, who passed on to me his interest for self-supervised learning. Wouter, I am very proud of the projects we did together. You are a very good researcher and a dedicated worker. I am thankful for our collaborations throughout the years!

I would also like to thank my other co-authors, Thierry Deruyttere, Dusan Grujicic, Davy Neven, Bert De Brabandere and Marc Proesmans. Thank you Thierry and Dusan for being great colleagues, for working long hours when we had a deadline and for all the fun discussions. Davy and Bert, it was nice to have you as my master thesis supervisors. I am happy we became colleagues and friends after! Marc, thank you for your endless feedback, for being a great listener and for all the times you joined me for a coffee break.

Further, I was also lucky to be surrounded by awesome office mates, Yu-Hui Huang, Yevhen Kuznietsov, Wouter Van Gansbeke and Liqian Ma. Our office certainly did not qualify as a standard working place as there were many distractions. Rare moments of quiet concentration were often interrupted by Yevhen, who wanted to share his opinion on something. I will certainly miss the fun moments we shared in the office. I would also like to thank Ali Diba - my office mate during my early days at Visics. Ali, thanks for passing on your knowledge and for all the fun talks we had!

Some of the nicer things about the PhD were the trips abroad - where we had some time to relax. I fondly remember the trip to Tokyo with Yu-Hui and Wouter - where we did plenty of sight-seeing, eating sushi and walking during our free time. Another great trip was the summer school in Sicily with Matthias, Thomas, Yevhen and Wouter. The lectures were alternated with swimming, playing volleyball and drinking Sicilian wine. 

I am also grateful for my other colleagues at Visics and Trace, who turn this place into a nice working environment: Matthias, Ali (2x), Dusan, Yu-Hui, Abhishek, Yevhen, Tim, Liqian, Xingchen, Nicola, Robby, Cedric, Gorjan, Soroush, Wouter, Thomas, Eli, Kaili, Bert (2x), Davy, Rahaf, Maxim, Klaas, Marc, Gioa, Bruno, Wim, Jonas, Michael, Mark, Aymen, Paul, Pattrica, Annitta,... Thanks for all the birthday cakes, the volleyball games, the beers at Oude Markt, etc. 

Finally, I reserve this part to thank some other important people in my life. My achievements would be both impossible and meaningless without them. Thank you to all my relatives and friends, the ones in Belgium, and the ones abroad. A special thanks goes to my friends from Roeselare: Arnaud, Dieter, Gilbert, Giel, Guillaume, Jan, Jens, Jos, Kenneth, Robin and Sam. I am very grateful for our friendship! A big thanks also goes to the people that turned Leuven into a wonderful place to live. I am thankful for all the people who became my friends during my time in Leuven. I won't forget our nights out! I would also like to thank Malou for bringing so much joy and happiness into my life. Thank you for always being there! Finally, the most special thanks goes to my parents - Stefaan and Carine - my brother - Maarten - and my other family members for their unconditional love and support. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/publications/publications.tex <==
\chapter{List of Publications}

\subsubsection{Articles in international peer reviewed conferences or journals}

(*) denotes equal contribution. 

\begin{itemize}
    \item Van Gansbeke, W.*, \textbf{Vandenhende, S.}*, Georgoulis, S., \& Van Gool, L. (2021). Revisiting Contrastive Methods for Unsupervised Learning of Visual Representations. In Conference on Neural Information Processing Systems.~\cite{van2021revisiting}
    \item Van Gansbeke, W.*, \textbf{Vandenhende, S.}*, Georgoulis, S., \& Van Gool, L. (2021). Unsupervised semantic segmentation by contrasting object mask proposals. In International Conference on Computer Vision.~\cite{van2021unsupervised}
    \item \textbf{Vandenhende, S.}, Georgoulis, S., Van Gansbeke, W., Proesmans, M., Dai, D., \& Van Gool, L. (2021). Multi-task learning for dense prediction tasks: A Survey. IEEE Transactions on Pattern Analysis and Machine Intelligence.~\cite{vandenhende2021multi}
    \item \textbf{Vandenhende, S.}, Georgoulis, S., De Brabandere, B., \& Van Gool, L. (2020) Branched Multi-Task Networks: Deciding What Layers To Share. In British Machine Vision Conference.~\cite{vandenhende2019branched}
    \item \textbf{Vandenhende, S.}, Georgoulis, S., \& Van Gool, L. (2020). Mti-net: Multi-scale task interaction networks for multi-task learning. In European Conference on Computer Vision.~\cite{vandenhende2020mti}
    \item Van Gansbeke, W.*, \textbf{Vandenhende, S.}*, Georgoulis, S., Proesmans, M., \& Van Gool, L. (2020). Scan: Learning to classify images without labels. In European Conference on Computer Vision.~\cite{van2020scan}
    \item Deruyttere, T., \textbf{Vandenhende, S.}, Grujicic, D., Van Gool, L., \& Moens, M. F. (2019). Talk2Car: Taking Control of Your Self-Driving Car. In Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP).~\cite{deruyttere2019talk2car}
    \item \textbf{Vandenhende, S.}, De Brabandere, B., Neven, D., \& Van Gool, L. (2019). A three-player GAN: generating hard samples to improve classification networks. In 2019 16th International Conference on Machine Vision Applications.~\cite{vandenhende2019three}
\end{itemize}

\subsubsection{Articles in international peer reviewed workshops}
\begin{itemize}
    \item Deruyttere, T., \textbf{Vandenhende, S.}, Grujicic, D., Liu, Y., Van Gool, L., Blaschko, M., ... \& Moens, M. F. (2020, August). Commands 4 Autonomous Vehicles (C4AV) Workshop Summary. In European Conference on Computer Vision.~\cite{deruyttere2020commands}
\end{itemize}

\subsubsection{Workshops}
\begin{itemize}
    \item Commands For Autonomous Vehicles Workshop (C4AV), ECCV, August, 2020.
    \item Workshop on Multi-Task Learning in Computer Vision (DeepMTL), ICCV, October, 2021.
\end{itemize}

\subsubsection{Awards}
\begin{itemize}
    \item Best paper award at the International Conference on Machine Vision Applications, Tokyo, May, 2019.
\end{itemize}
